Deep Dependency Networks and Advanced Inference Schemes for Multi-Label Classification

We present a unified framework called deep dependency networks (DDNs) that combines dependency networks and deep learning architectures for multi-label classification, with a particular emphasis on image and video data. The primary advantage of dependency networks is their ease of training, in contrast to other probabilistic graphical models like Markov networks. In particular, when combined with deep learning architectures, they provide an intuitive, easy-to-use loss function for multi-label classification. A drawback of DDNs compared to Markov networks is their lack of advanced inference schemes, necessitating the use of Gibbs sampling. To address this challenge, we propose novel inference schemes based on local search and integer linear programming for computing the most likely assignment to the labels given observations. We evaluate our novel methods on three video datasets (Charades, TACoS, Wetlab) and three image datasets (MS-COCO, PASCAL VOC, NUS-WIDE), comparing their performance with (a) basic neural architectures and (b) neural architectures combined with Markov networks equipped with advanced inference and learning techniques. Our results demonstrate the superiority of our new DDN methods over the two competing approaches.

==> content/1-intro.tex <==


In this paper, we focus on the multi-label classification (MLC) task, and more specifically, on its two notable instantiations, multi-label action classification (MLAC) for videos and multi-label image classification (MLIC). At a high level, given a pre-defined set of labels (or actions) and a test example (video or image), the goal is to assign each test example to a subset of labels.
It is well known that MLC is notoriously difficult because, in practice, the labels are often correlated, and thus predicting them independently may lead to significant errors. Therefore, most advanced methods explicitly model the relationship or dependencies between the labels, using either probabilistic techniques \cite{wang2008generative,rossiProceedingsTwentyThirdInternational2013b, antonucci2013ensemble, wangEnhancingMultilabelClassification2014a, Tan_2015_CVPR,pmlr-v52-dimauro16} or non-probabilistic/neural methods  \cite{kongMultilabelClassificationMining2013a,papagiannopoulouDiscoveringExploitingDeterministic2015a,chenLearningSemanticSpecificGraph2019,chenMultiLabelImageRecognition2019,wang2021semi,nguyenModularGraphTransformer2021,wangNovelReasoningMechanism2021a,liuQuery2LabelSimpleTransformer2021, quMultilayeredSemanticRepresentation2021,liu_2022_text,zhou_2023_double, weng_2023_learning}. 


\eat{To this end, motivated by approaches that combine probabilistic graphical models (PGMs) with neural networks (NNs)  \cite{krishnanDeepKalmanFilters2015, johnsonComposingGraphicalModels2017}, as a starting point, we investigated using (Conditional) Markov random fields (CRFs and MRFs), a type of undirected PGM, to capture the relationship between the labels as well as those between the labels and features derived from feature extractors. Unlike previous work, which used these MRF+NN or CRF+NN hybrids with conventional inference schemes such as Gibbs sampling (GS) and mean-field inference, our goal was to evaluate whether \textit{advanced approaches}, specifically (1) iterative join graph propagation (IJGP) \cite{mateescu2010join}, a type of generalization Belief propagation technique \cite{yedidiaGeneralizedBeliefPropagation2000}, (2) integer linear programming (ILP) based techniques for computing most probable explanations and (3) a well-known structure learning method based on logistic regression with $\ell_1$-regularization \cite{NIPS2006_lee_a4380923,NIPS2006_Wainwright_86b20716}, can improve the generalization performance of MRF+NN hybrids.} 

\old{To measure and compare performance of these MRF+NN hybrids with NN models, we used several metrics such as mean average precision (mAP), label ranking average precision (LRAP), subset accuracy (SA), and the jaccard index (JI) and experimented on three video datasets: (1) Charades \cite{charades_paper}, (2) TACoS \cite{tacos:regnerietal:tacl} and (3) Wetlab \cite{wetlab:Naim2014UnsupervisedAO} and three image datasets: (1) MS-COCO \cite{linMicrosoftCOCOCommon2015}, (2) PASCAL VOC 2007 \cite{everinghamPascalVisualObject2010} and (3) NUS-WIDE \cite{chuaNUSWIDERealworldWeb2009a}. We found that generally speaking, both IJGP and ILP are superior to the baseline NN and Gibbs sampling in terms of JI and SA but are sometimes inferior to the NN in terms of mAP and LRAP. We speculated that because MRF structure learners only allow pairwise relationships and impose sparsity or low-treewidth constraints for faster, accurate inference, they often yield poor posterior probability estimates in high-dimensional settings. Since both mAP and LRAP require good posterior probability estimates, GS, IJGP, and ILP exhibit poor performance when mAP and LRAP are used to evaluate the performance.}


\old{
To circumvent this issue and in particular to derive good posterior estimates, we propose a new PGM+NN hybrid called \textit{deep dependency networks} (DDNs). At a high level, a dependency network (DN) \cite{heckerman2000dependency} represents a joint probability distribution using a collection of conditional distributions, each defined over a variable (label) given all other variables (labels) in the network. Because each conditional distribution can be trained locally, DNs are easy to train. However, a caveat is that they are limited to Gibbs sampling for inference and are not amenable to advanced probabilistic inference techniques \cite{lowdClosedFormLearningMarkov2012a}.
}

 %such as an image or video segment,
\sva{To this end, motivated by approaches that combine probabilistic graphical models (PGMs) with neural networks (NNs)  \cite{krishnanDeepKalmanFilters2015, johnsonComposingGraphicalModels2017}, we jointly train a hybrid model, termed \textit{deep dependency networks} (DDNs) \cite{guo_2020_deep}, as illustrated in Figure \ref{fig:ddn_intro}. In a Deep Dependency Network (DDN), a conditional dependency network sits on top of a neural network. The underlying neural network transforms input data (e.g., an image) into a feature set. The dependency network \cite{heckerman2000dependency} then utilizes these features to establish a local conditional distribution for each label, considering not only the features but also the other labels. \eat{This architecture thus combines the feature extraction capabilities of neural networks with the probabilistic modeling proficiency of dependency networks \cite{heckerman2000dependency}.}

However, a limitation of DDNs is that they rely on basic methods like Gibbs sampling and mean-field inference for probabilistic reasoning, and lack advanced probabilistic inference techniques \cite{lowd_2011_mean,lowdClosedFormLearningMarkov2012a}. This paper addresses these limitations by introducing sophisticated inference schemes tailored for the Most Probable Explanation (MPE) task in DDNs, which involves finding the most likely assignment to the unobserved variables given observations. In essence, a solution to the MPE task, when applied to a probabilistic model defined over labels and observed variables, effectively solves the multi-label classification problem.

More specifically, we propose two new methods for MPE inference in DDNs. Our first method uses a random-walk based local search algorithm. Our second approach uses a piece-wise approximation of the log-sigmoid function to convert the non-linear MPE inference problem in DDNs into an integer linear programming problem. The latter can then be solved using off-the-shelf commercial solvers such as Gurobi \cite{gurobi}.


%However, a caveat is that DDNs are limited to Gibbs sampling \cite{heckerman2000dependency} and mean-field inference \cite{lowd_2011_mean} and are not amenable to advanced probabilistic inference techniques \cite{lowdClosedFormLearningMarkov2012a}. To address these shortcomings, this paper presents \textit{sophisticated} inference schemes designed specifically for the Most Probable Explanation (MPE) task in DDNs. Initially, we propose utilizing local search-based algorithms, specifically random walk and greedy search, as an initial strategy for addressing this task. 
\eat{In the random walk approach, the model randomly perturbs the input value for each iteration. In contrast, the greedy technique selects and adjusts the variable that yields the highest score for the succeeding sample.}

%Furthermore, we introduce a novel method for MPE in DDNs. This approach optimizes an objective function specifically designed for MPE while enforcing constraints for precise DN representation. It accommodates the inclusion of multiple constraints, thereby facilitating the integration of prior knowledge concerning both the inputs and outputs into the optimization algorithm. The deterministic nature of our proposed approach stands out as its unique attribute, effectively countering the variabilities induced by random initializations observed in various sampling and search methodologies. The implementation of these methods has two significant advantages: enhanced probabilistic inference in DDNs, and the availability of a broader range of techniques for MPE within these networks.
}

% \icml{We again use the various models mentioned above to extract the features for the PGM. \eat{This helps us to show that the DDN model does not depend on the type of the feature extractor selected and it can improve the performance on top of different types of any architectures.}}
\begin{figure}[t]%{l}{.5\textwidth}
\vskip 0.2in
        \begin{center}
        \centerline{\includegraphics[width=0.99\columnwidth]{images/dn_intro.pdf}}
        \caption{Illustration of improvements made by our proposed inference scheme for DDNs. The DDN learns label relationships and the inference scheme excels in leveraging these relationships to accurately identify concealed objects, such as the \textbf{sports ball}.}
        \label{fig:ddn_intro}
        \end{center}
\vspace{-8mm}
\end{figure}

We evaluate DDNs equipped with our new MPE inference schemes and trained via joint learning on three video datasets: Charades \cite{charades_paper}, TACoS \cite{tacos:regnerietal:tacl}, and Wetlab \cite{wetlab:Naim2014UnsupervisedAO}, and three image datasets: MS-COCO \cite{linMicrosoftCOCOCommon2015}, PASCAL VOC 2007 \cite{everinghamPascalVisualObject2010}, and NUS-WIDE \cite{chuaNUSWIDERealworldWeb2009a}. We compare their performance to two categories of models: (a) basic neural networks (without dependency networks) and (b) hybrids of conditional random fields (CRFs), an undirected PGM, and neural networks equipped with sophisticated reasoning and learning algorithms.  Specifically, we employ three advanced approaches: : (1) iterative join graph propagation (IJGP) \cite{mateescu2010join}, a type of generalization Belief propagation technique \cite{yedidiaGeneralizedBeliefPropagation2000} for marginal inference, (2) integer linear programming (ILP) based techniques for computing most probable explanations (MPE) and (3) a well-known structure learning method based on logistic regression with $\ell_1$-regularization \cite{NIPS2006_lee_a4380923,NIPS2006_Wainwright_86b20716} for learning the structure of pairwise conditional random fields (CRFs).


%\sva{Subsequently, we investigated employing Conditional Markov Random Fields (CRFs and MRFs) as undirected Probabilistic Graphical Models (PGMs) to serve as a comparative baseline in hybrid architectures. Unlike previous work, which used these MRF+NN or CRF+NN hybrids with conventional inference schemes such as Gibbs sampling (GS) and mean-field inference, our goal was to evaluate whether \textit{advanced approaches}, specifically (1) iterative join graph propagation (IJGP) \cite{mateescu2010join}, a type of generalization Belief propagation technique \cite{yedidiaGeneralizedBeliefPropagation2000}, (2) integer linear programming (ILP) based techniques for computing most probable explanations and (3) a well-known structure learning method based on logistic regression with $\ell_1$-regularization \cite{NIPS2006_lee_a4380923,NIPS2006_Wainwright_86b20716}, can improve the generalization performance of MRF+NN hybrids.
%}

\old{In our proposed deep dependency network (DDN) architecture, a dependency network sits on top of a feature extractor based on a neural network. We illustrate the workings of the DDN architecture in Figure \ref{fig:ddn_intro}. The feature extractor converts the input image or video segment to a set of features, and the dependency network uses these features to define a local conditional distribution over each label given the features and other labels. We show that deep dependency models are easy to train either jointly or via a pipeline method where the feature extractor is trained first, followed by the DNN by defining an appropriate loss function that minimizes the negative pseudo log-likelihood \cite{besag_statistical_1975} of the data. 
We conjecture that because DDNs can be quite dense, they often learn a better representation of the data, and as a result, they are likely to outperform MRFs learned from data in terms of posterior predictions.}

\old{We found that, generally speaking, for MRF+NN (DRF) both IJGP and ILP are superior to the baseline NN and Gibbs sampling in terms of JI and SA but are sometimes inferior to the NN in terms of mAP and LRAP. We speculated that because MRF structure learners only allow pairwise relationships and impose sparsity or low-treewidth constraints for faster, accurate inference, they often yield poor posterior probability estimates in high-dimensional settings. Since both mAP and LRAP require good posterior probability estimates, GS, IJGP, and ILP exhibit poor performance when mAP and LRAP are used to evaluate the performance.

We trained DDNs using the joint learning approach and evaluated them using the four aforementioned metrics and six datasets. We observed that jointly trained DDNs are often superior to the baseline neural networks as well as advanced MRF+NN methods that use GS, IJGP, and ILP on all four metrics. Specifically, they achieve the highest scores on all metrics on five out of the six datasets. Also, we found that the jointly trained DDNs are more accurate than the ones trained using the pipeline approach. This is because end-to-end (or joint) learning steers the feature selection process to provide tailored features for the DN, and learns a DN that is in-turn tailored to the output of this backbone. DDNs provide a multi-label classification head that works on the features extracted by the backbone.}

The experimental setup involved the assessment of the proposed methods on three video datasets: Charades \cite{charades_paper}, TACoS \cite{tacos:regnerietal:tacl}, and Wetlab \cite{wetlab:Naim2014UnsupervisedAO}, alongside three image datasets: MS-COCO \cite{linMicrosoftCOCOCommon2015}, PASCAL VOC 2007 \cite{everinghamPascalVisualObject2010}, and NUS-WIDE \cite{chuaNUSWIDERealworldWeb2009a}.
\sva{Given the emphasis on the MPE tasks, which solely focuses on label assignments, the utilization of mean average precision (mAP) as a metric for evaluation is inappropriate\footnote{Although mAP is a conventional metric for MLC, its applicability is restricted in this context.}. Consequently, we limited our evaluation to the use of Subset Accuracy (SA) and Jaccard Index (JI) for the evaluation of MRF+NN hybrids and various DDN inference strategies, which are more appropriate metrics for the MPE task.




Our evaluations have consistently demonstrated the superiority of MRF+NN hybrids that incorporate IJGP and ILP over baseline NNs and Gibbs sampling in terms of both Jaccard Index (JI) and Subset Accuracy (SA). However, the structural limitations of MRFs, which only permit pairwise relationships and require sparsity for efficient inference, may hinder the performance of PGM+NN. Therefore, it may be beneficial to explore alternative models such as DDNs, which are better equipped to capture label interdependencies.

The optimization-focused MPE inference approach for DDNs demonstrated superior performance compared to standard neural networks and advanced MRF+NN inference schemes, as evidenced by its consistent outcomes in multiple evaluation metrics. Furthermore, it exhibits a clear advantage over existing sampling and search-based inference techniques specifically tailored for DDNs. As a result, the proposed strategy achieved superior performance on four of the six evaluated datasets.}


\eat{We implemented DDNs in PyTorch and the code implementation to reproduce our experiments is available here\footnote{We provide the implementation of DDN at \url{https://anonymous.4open.science/r/DDN-C3B9}} and will be later published on GitHub.
}

%

\eat{
We evaluated DDNs using the four aforementioned metrics and six datasets. We observed that they are often superior to the baseline neural networks as well as MRF+NN methods that use GS, IJGP, and ILP on all four metrics. 
% Specifically, they achieve the highest score on the SA and JI metrics on all the datasets while having higher or competitive mAP scores. 
Specifically, they achieve the highest score on all metrics on five out of the six datasets and kept a comparable mAP score while improving on SA and JI metrics for the remaining dataset. 
\icml{Subset accuracy is a really important metric for situations where an exact match is required between the predictions and true labels. For example, in symptom detection in the medical domain and image classification in autonomous vehicles. Thus various methods\cite{dembczynskiBayesOptimalMultilabel,namMaximizingSubsetAccuracy2017,NEURIPS2021_859bf141} have been proposed for the task of exact multi-label classification (E-MLC) that optimize their models on subset accuracy.
Subset Accuracy is a very harsh metric since it completely ignores partially correct predictions; impressively, the proposed method improved the metric by as much as 34\% even though it was not trying to optimize for subset accuracy.}
We compared the pipeline model with the jointly learned model and found that the joint model is more accurate than the pipeline model. End-to-end learning steers the feature selection process to provide tailored features for the DN, and a DN that is in-turn tailored to the output of this backbone. \icml{DDNs work as a multi-label classification head that works on the features extracted by the backbone.}We also show that DDNs can improve on state-of-the-art methods that already model the above-mentioned relationships, suggesting that DDNs can model additional relationships missed by these methods.
}
% \eat{Specifically, they achieve the highest score on the mAP metric on all the datasets.} 

In summary, this paper makes the following contributions:
\begin{itemize}
    \eat{\item \sva{We propose the use of sophisticated training and inference techniques to enhance the generalization capabilities of MRF+NN hybrid models.} \sva{Not sure if we should add this or not but we say in the paper that there is no other work that has used these advanced methods for MRFs+DDNs}}
    \item We jointly train a hybrid model called deep dependency networks that combines the strengths of dependency networks (faster training and access to probabilistic inference schemes) and neural networks (flexibility, high-quality feature representation).
    % \item \sva{Are we defining a new loss function now? When we just use a single loss (from the DN)} We define a new loss function for jointly training the neural and dependency network components of the deep dependency network. We show that DDNs are easy to train using these loss functions.
    \item \sva{We present novel inference methodologies tailored for the MPE task in Dependency Networks (DNs). Contrary to traditional approaches that predominantly utilize Gibbs Sampling, our proposed method enhances the task's effectiveness, delivering superior outcomes in a shorter computational period.
    \item We carried out a series of experiments utilizing the proposed inference schemes on a total of six datasets, consisting of three videos and three images, to address multi-label action and image classification tasks using two metrics. Our results were compared against those obtained using baseline NN, MRF+NN methods and alternative inference schemes.}  %We found that jointly trained DDNs consistently outperform NNs and MRF+NN hybrids on all metrics and datasets. %We also show that DDNs can improve on state-of-the-art methods that already model the above-mentioned relationships, suggesting that DDNs can model additional relationships missed by these methods.
\end{itemize}



%\todo{Describe dependency nets, how learning them is easy and issues. Then describe how to do joint learning with dnns and cnns. } 


% Why are we using CNNs as feature extractors, and how can PGMs be used for these features 
%\eat{
%Convolutional Neural Networks have been popular feature extractors for various visual inputs \cite{razavianCNNFeaturesOfftheshelf2014, govindaswamyCNNFeatureExtractor2020, guerinCombiningPretrainedCNN2021, joginFeatureExtractionUsing2018, teodoroAnalysisImageFeatures2021}. The features extracted by the CNN can be used by other models to perform the prediction/classification task. Probabilistic Graphical Models (PGMs) have often been used to process these extracted features and produce the outputs for various deep models. Some of the examples where these kinds of models being used are as follows - image crowd counting \cite{hanImageCrowdCounting2017}, structured output prediction \cite{pmlr-doNeuralConditionalRandom2010}, visual relationship detection \cite{yuProbabilisticGraphicalModel_2022_CVPR}, modeling for epileptic seizure detection in multichannel EEG \cite{craleyIntegratingConvolutionalNeural2019a}, phonetic recognition \cite{morrisConditionalRandomFields2008}, Face Sketch Synthesis \cite{zhangNeuralProbabilisticGraphical2020}, semantic image segmentation \cite{chenDeepLabSemanticImage2018, linEfficientPiecewiseTraining2015}, animal pose tracking \cite{wuDeepGraphPoseNEURIPS2020}, pose estimation \cite{chenArticulatedPoseEstimation2014} and Adaptive Team Training \cite{rollArtificialIntelligenceEducation2021}. Furthermore, based on these examples, we can say that using PGMs to process the features extracted from CNN can be a great way to tackle various tasks where there is a relationship between the features and outputs. 
%One example of the use of PGMs to model these inter-label dependencies can be a case when a person is performing the task of getting something from a cupboard. First, they need to open the cupboard (if it is already not open), take the item, and then close it. It might happen that the deep neural network might not be able to detect one of these actions. However, we can use a PGM to utilize the relationships between these activities and predict that the un-detected activity was performed.
%}

% Why MRFs and DNs
\eat{Motivated by the existing approaches that combine DNNs with PGMs, we will use DNNs to extract features and PGMs to process these features and model the relationships between the output labels from DNNs. Dependency Networks \cite{heckerman2000dependency} are graphical models represented by a set of conditional probability distributions. They have been proposed as alternatives to other PGMs like Bayesian Networks and Markov Networks due to their faster learning algorithms. The learning process can also be parallelized, which makes learning even faster. They can also be cyclic, which is not the case for Bayesian Networks. The only issue with DNs is that we cannot apply the inference techniques proposed for other PGMs, and we have to resort to Gibbs sampling for inference. 
Dependency Networks model the distributions of a given variable using all the other variables, thus giving a computationally efficient way of learning the required distributions. Another probabilistic model we can use to represent these dependencies is Markov Random Field (MRFs). MRFs are undirected graphs that also allow cycles. The only issue with using MRFs is that the inference would become intractable \cite{rothHardnessApproximateReasoning1996} if the treewidth is not bounded. Thus we need to add constraints to the Markov blanket for the nodes to make the inference possible.
\eat{Learning structure and parameters of MRFs is challenging due to the presence of the normalizing factor in the distribution equation. Therefore, many approximations have been proposed to perform this task, which is faster but might not give the best possible models.} 
Moreover, we are not bound to the task of multi-label activity classification since we are learning the model structures and parameters. By using these PGMs, we can model the label-label and feature-label relationships, thus making them a perfect choice to be really good at multi-label classification.  

% \eat{For both models, the features are extracted by a Convolutional Neural Network, and a PGM is used to process these features. We have a Markov Random Field as the PGM for the first model. While in the second model, we have a Dependency Network as the PGM, which improves on the results of the first model.}

This paper addresses the challenges mentioned above by using the two proposed models. \yu{I do not see what are the challenges.} We choose these two as PGMs because they allow cycles in their graphs, which can thus be used to represent cyclic dependencies and help tackle the multi-label classification task. \yu{By two PGMs, do you mean dependency networks and MRFs?} We will learn the structure and distributions of both the models from data, thus making it an extensive method and allowing the proposed learning and inference processes to be used for various tasks. Once the models are learned, we will use various inference techniques, including Iterative Join Graph Propagation (IJGP) \cite{mateescu2010join}, Integer Linear Programming (ILP) \cite{wainwright2008graphical} for the Markov Random Field, and Gibbs Sampling \cite{sacco1990stochastic} for the Dependency Network to infer the class labels. After this, we will jointly train the Dependency Network with the Convolutional Neural Network to improve the learned representations even more. As such, we dub this approach Deep Dependency Networks. Based on our results, it can be concluded that learning better representation can outperform more sophisticated inference techniques. The proposed models are easy to train and have a small overhead on top of the feature extractor and provide a significant improvement. Experiments on three datasets will be performed to show the improvements of the proposed methods over the baseline. The patterns in the evaluation metrics for various datasets show that learning better representations of the data (learned in Dependency Networks) can perform better than using more sophisticated inference techniques (used for inference in MRFs) for the case of PGMs. This can be because MRFs do not perform very well in high dimensions, i.e., when the number of nodes increases in an MRF, the inference task becomes more complex, and even approximate algorithms do not provide reasonable estimates. \yu{This paragraph needs to be improved. Not very clear about the contributions.} 

One thing that needs to be pointed out here is that we propose to use CNNs to extract features; however, other feature extractors can also be used, and the proposed model does not depend on the type of feature extractor. Furthermore, this method is proposed to solve the task of multi-label activity recognition. However, it is not bound to this task and thus can also be used for other multi-label classification tasks.
}




==> content/4-model.tex <==
\subsection{Inputs to the PGM}
The output of the classification layer will be treated as the features extracted from the Convolutional Neural Network; thus, the size of this feature vector will be (1, number of true labels) for each instance. 
%The reason behind this is that it helps us model the relationships between these labels and the labels that the PGM will predict.
By using these features we fulfill two tasks at once. Firstly we can utilize the information extracted by the NNs and also model the relationships between the true labels and the output probabilities of the CNN. For example high feature probability for an activity open cupboard can help the model to interpret that it can be either open cupboard or close cupboard, since both these labels have similar kind of examples in the video. These relationships can be learned by PGMs and thus help in improving the model performance. 
In addition to this information, we can also use the inter-label dependencies to predict the final output. 
Thus the nodes in the PGMs will be of two types - $\displaystyle \rve$ and $\displaystyle \rvy$. The nodes $\displaystyle \rvy$ will correspond to the output labels that will be inferred from the PGM. Furthermore, $\displaystyle \rve$ nodes will represent the evidence we get from the CNN. Thus we will define a PGM over the graph $\displaystyle \gG$ whose nodes will be  $\displaystyle \sX = (y_1,....., y_n, x_1,.....,x_n)$ where n is the total number of labels in the given dataset. 


\subsection{Markov Random Fields}
\subsubsection{Structure Learning}
We will define a joint distribution over all the variables in $\displaystyle \rvy$ and $\displaystyle \rve$. For each node $\displaystyle y_i$ its neighbors will be ($\displaystyle \sN(y_i), x_i$). Where $\displaystyle \sN(y_i) \subseteq (y_1, ..... , y_{i-1}, y_{i+1}, ...... , y_{n})$. For structure learning of the MRF we will use $\displaystyle L_1$-regularized logistic regression \cite{NIPS2006_86b20716, NIPS2006_a4380923}, to get the set $\sN(y_i)$ for each $\displaystyle y_i$. $\displaystyle \sN(y_i)$ is also called Markov blanket of the node $y_i$. We have provided an example of how the MRF would look in Figure \ref{fig:pgm_lr_dn} where $\displaystyle \sN(y_1) = y_2, \sN(y_2) = (y_1, y_3), \sN(y_3) = y_2 $. This method helps us find the set of nodes highly related to the given node to create the neighborhood and thus include important relationships in the graph. The only issue with MRFs is that we need to bound the number of neighbors for each node in the graph; otherwise, if the graph is too densely connected, inference tasks in MRFs become hard for exact inference. Approximate inference techniques also become less accurate, thus getting poorer results. Thus for these experiments, we learn MRFs with neighborhood size capped by 10. 

\subsubsection{Parameter Learning}
We learn the parameters of the MRF by using Maximum Pseudo-likelihood Parameter Estimation \cite{koller2009probabilistic}. We do not use Likelihood Parameter Estimation because it requires running inference over the network in each iteration, making the learning process very slow. However, that is not the case if we use Pseudo-likelihood as the training objective. Furthermore, the inference becomes even slower if the model has a high tree width. We use L2 regularization with stochastic gradient descent to learn the parameters of the MRF so that the model does not over-fit the data. In many cases, pseudo-likelihood as an objective can perform very well, reducing the computational cost of learning. Pseudo-likelihood can be defined as follows
\begin{equation}
\displaystyle l_{P L}(\theta: \mathcal{D})=\frac{1}{M} \sum_{m=1}^M \sum_{j=1}^n \ln p \left(x_{j}[m] \mid x_{-j}[m], \boldsymbol{\theta}\right)
\end{equation}
where $\displaystyle \theta$ is the model's parameters, $\displaystyle M$ is the number of examples in dataset $\displaystyle \mathcal{D}$, and $\displaystyle n$ is the number of variables in the model. 

\subsubsection{Inference}
We will perform two different tasks for inference, maximum a posteriori (MAP) estimation task using Integer Linear Programming solver and Belief Update task using Iterative Join-Graph Propagation (IJGP) solver. MAP inference can be defined as assigning the most probable values to the variables in a graph, given the evidence. Finding the MAP assignment is an NP-hard task unless we are given tree-structured graphs or graphs with bounded tree-width \cite{dechter2003constraint, globersonFixingMaxProductConvergent}. Belief Update is the task where we compute the posterior probability $\displaystyle P(Y|e)$ where $\displaystyle Y$ are the query nodes, and $e$ is the given evidence. IJGP is an iterative version of join-tree clustering that can be used as a generalized belief propagation method. Thus we are performing two tasks, one that provides us with the assignment to the variables and one that outputs the probabilities of the query nodes given the evidence. These two sophisticated inference techniques for MRFs perform well for the corresponding tasks.  


\subsection{Conditional Dependency Networks}

\yu{We need to present Deep Dependency Networks in the method section.}

\subsubsection{Structure Learning}
We will use the conditional dependency networks proposed in \cite{guo2011multi} that have been proved to model the inter-label dependencies for the multi-label classification task. For this model, we will define a conditional joint distribution over all the variables in $\displaystyle \rvy$, assuming that the evidence variables $\displaystyle \rve$ are given, and this evidence comes from CNN. For each node $\displaystyle y_i$ its parent set will be $\displaystyle \parents_\gG(y_i) = \{y_{-i}, x\}$ and the distribution $\displaystyle \gP$ will be defined only on the $\displaystyle \rvy$ variables, being conditioned on $\displaystyle \rve$. By doing this, we will get a model where the Markov blanket (MB) of each node will be all the other label nodes($\displaystyle y_{-i}$) and all the feature nodes ($\displaystyle \rve$). We have provided an example of how the DN would look in Figure \ref{fig:pgm_lr_dn}. We use two models to define the conditional probability distributions in $\displaystyle \gP$; the first is a logistic regression (LR) model. Representing dependency networks using logistic regression was proposed in \citet{heckerman2000dependency}. Since Neural Networks have been proved to have more representation power than the Logistic Regression model, we will also represent each distribution using a NN. 

\subsubsection{Parameter Learning}
For both the models, we will learn the parameters by minimizing the Cross-Entropy loss on the output variable of the model, using stochastic gradient descent. For the logistic regression model, we use L1 regularization to learn the Markov blanket of the node and thus only choose nodes that help predict the output node. We use regularization for both models to stop them from overfitting. While training, the input to the model that predicts $\displaystyle y_{i}$ will be a vector that is the concatenation of $\displaystyle y_{-i}$ and $\displaystyle x$, and we will have n of these models, each for a $\displaystyle y_{i}$. Since each of the models representing the distribution of a different $\displaystyle y_{i}$ are not dependent on each other, we can train them in parallel, thus making the learning process very fast. We also implemented both the models in PyTorch, which helps us to use GPUs while training making it even faster. 


\subsubsection{Inference}
We will use a Systematic-Scan Gibbs Sampling to perform the inference for Dependency Networks. There is a possibility that Dependency Networks may not model a probability distribution. However, \citet{heckerman2000dependency} has argued that if the number of samples is large enough during inference, then the distribution of the outputs provided by the Gibbs sampler is consistent with a conditional distribution. Since cycles are also allowed in Dependency Networks, we cannot use inference methods that can be used with Bayesian Networks and Markov Networks, like Variable Elimination and  Iterative Joint Graph Propagation. 



To estimate the marginal probabilities of the output variable, we will use \textbf{Mixture Estimator}, which is defined in \ref{Mixture_Estimator}
$$
\label{Mixture_Estimator}
\displaystyle \hat{P}\left(x_{i}\right)=\frac{1}{N} \sum_{j=1}^{N} P\left(x_{i}^{(j)} \mid \textbf{x}_{MB(X_{i})}^{(j)}\right)
$$
where $\displaystyle x_i$ is the node for which we want to find the probabilities and $\displaystyle \textbf{x}_{MB(x_{i})}$ is the Markov blanket of the variable $\displaystyle x_i$. The variable $\displaystyle j$ goes over the examples. 
\begin{figure}
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width= 0.98\textwidth]{icml2023/images/dn.pdf}
        \caption{Dependency Network Structure}
    \end{subfigure}\hfill
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width= 0.98\textwidth]{icml2022/images/mrf.pdf}
        \caption{Markov Random Field Structure}
    \end{subfigure}
    \caption{Probabilistic Graphical Models}
    \label{fig:pgm_lr_dn}
\end{figure}

% \begin{frame}
% \frametitle{Systematic-Scan Gibbs Sampler}
% The Systematic-Scan Gibbs Sampler algorithm is given by\\
% \begin{enumerate}
%     \item Sample s = Random assignment to $\forall X_i$ nodes. \\
%     \textbf{Iterate till convergence or fixed number of iterations:}
% \\
% For iteration t+1
% \\
% For all i = 1,....,n 
%      \begin{enumerate}
%             \item Sample $(X_i^{(t+1)} = x_i)$ from $P(X_{i} \mid x_{1}^{(t+1)},...,x_{i-1}^{(t+1)},x_{i+1}^{t},...,x_{n}^{t},e_{1}^{(t+1)},...,e_{n}^{(t+1)})$
%             \item Replace $(X_i = x_i)$ in Sample s
%         \end{enumerate}
% \end{enumerate}
% \end{frame}
% \begin{frame}


\eat{The Systematic-Scan Gibbs Sampler algorithm can be performed as given in Algorithm \ref{alg:gibbs_alg}
\begin{algorithm}
\caption{Systematic-Scan Gibbs Sampling}
\begin{algorithmic}
\Procedure{Gibbs Sampling}{$s, num\_iter$} 
\Comment{Sample s = Random assignment to $\forall X_i$ nodes.}
\State $t \gets 0$
\While{$t \leq num\_iter$}
\State $t \gets t + 1$
\State $i \gets 0$
% For iteration t+1
\While{$i \leq n$}
            \State $t \gets t + 1$
            \State Sample $(Y_i^{(t)} = Y_i)$ from $P(y_{i} \mid y_{1}^{(t)},..,y_{i-1}^{(t)},y_{i+1}^{t-1},..,y_{n}^{t-1},e_{1}^{(t)},..,e_{n}^{(t)})$
            \State Replace $(Y_i = y_i)$ in Sample s
\EndWhile
\EndWhile
\EndProcedure
\end{algorithmic}
\label{alg:gibbs_alg}
\end{algorithm}}

% WHY WE DO NOT USE GNNs TO MODEL LABEL DEPENDENCIES



==> content/5-Joint-learning.tex <==
\yu{Joint training is only for DN right? This section looks like for both MRF and DN.}

To do joint training, we need to select appropriate loss functions defined over the parameters of all the corresponding models and then perform gradient descent to minimize this loss. We use two losses to train the joint model \textemdash the first loss function is the Binary Cross Entropy ($\displaystyle BCE_{cnn}$) loss applied to the outputs of the CNN and true labels. The second loss function is the same as before; however, it is applied to the outputs of all the models representing the conditional probability distributions of the DNs. The loss ($\displaystyle BCE_{dn}$) will be applied to the output predicted by the $i^{th}$ model in the dependency network, $\displaystyle \hat{y_i}$ and the  $i^{th}$ true label $\displaystyle \vy_i$. Thus for the joint model, we will have $(N+1)$ losses where N is the total number of true labels in the given dataset. 

To start the end-to-end training process, we perform the forward pass on the CNN by providing the clip/frame input. After the getting the outputs of the CNN, we can calculate $\displaystyle BCE_{cnn}(\hat{Y}, Y_{cnn})$. Moreover, since we already have the values of the final layer of the CNN, we can now do the forward pass for the DN. Then we calculate $\displaystyle BCE_{dn}(\hat{Y}_{(i)}, Y_{dn^{(i)}})$ for each model of the DN. The loss $\displaystyle L_{joint}$, given in equation \ref{eq:cnn_joint_loss} is the resulting joint objective function, and it will be used to update the parameters of the two models using stochastic gradient descent. We do the same things for both the DN models, NN and LR; the only thing that changes is how we calculate the $\displaystyle BCE_{dn}^{(i)}$ and back-propagate its gradient through the models. 

\begin{equation}
\label{eq:cnn_joint_loss}
L_{joint} = BCE_{cnn}\left( \hat{Y}, Y_{cnn}\right) + \frac{1}{N} \sum_{i=1}^{N} BCE_{dn}\left( \hat{Y}_{(i)}, Y_{dn^{(i)}}\right)
\end{equation}

For the proposed model, the number of conditional distributions in the dependency networks depends on the number of true labels in the classes. This can become an enormous overhead over the feature extractor for datasets with an enormous number of labels (activities) since this model will require too much GPU memory if we try to run all the models in parallel. Thus to alleviate this problem, we optimize the joint loss by only allowing a fixed number of DN forward and backward passes simultaneously. Furthermore, the number of concurrent passes can be increased if required. We make this work by storing the gradients corresponding to the outputs of the NN until all the passes are finished, and then we can back-propagate the gradients through the NN. After training the model, the inference process remains the same as the previously mentioned pipeline model. Thus this joint learning process only adds overhead while training and provides with moderate to good improvements in the model performance. 

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=\textwidth]{icml2022/images/joint_back_prop.pdf}
\caption{Illustration of the joint learning process. Blue arrows represent forward pass. Red arrows represent backward pass}
\end{center}
\end{figure}

\eat{Now we will look at how to train the Dependency Network and CNN jointly. Firstly, we have two losses for the joint model; the first is Binary Cross Entropy ($\displaystyle BCE_{cnn}$) loss which is applied to the outputs of the CNN and true labels. The second loss ($\displaystyle BCE_{dn}$) is also the Cross-Entropy loss. However, it is applied to the outputs of all the Dependency Networks and their corresponding true labels separately. Thus for a network predicting $\displaystyle y_i$ the loss ($\displaystyle BCE_{dn}^{(i)}$) will be applied to the predicted output $\displaystyle \hat{y_i}$ and the true label $\displaystyle \vy_i$.} 

\eat{For the training iteration, we first do the forward pass on CNN by providing the clip/frame as input. After the forward pass through the CNN, we can calculate $\displaystyle BCE_{cnn}$. Moreover, since we already have the values of the final layer of the CNN, we can now do the forward pass for the DN by providing the concatenation of the true labels and outputs of the CNN as the input. Then we calculate $\displaystyle BCE_{dn}$ for all the DNs and back-propagate the gradients. To get the gradients for the CNN, we will first take the average of all the losses of the DNs ($\displaystyle \frac{1}{n} \sum_{i=1}^n BCE_{dn}^{(i)}$) and then add it to $\displaystyle BCE_{cnn}$. Since the inputs of the DNs are the outputs of the final layer of the CNN, the CNN and DN will be connected, and thus the loss corresponding to the DNs also depends on the variables in the CNN. Finally, these gradients are back-propagated through CNN. Thus the both the models are learned jointly and it helps to improve the performance over the pipeline model. }


==> content/9-future-work.tex <==
\eat{As we have mentioned before for some cases dependency networks might not correspond to valid distributions. Thus we cannot use more sophisticated inference techniques, that have been proposed for other probabilistic models, on dependency networks. But as we saw in this paper, learning better representations can be better than using more extensive inference techniques. What if we can use these sophisticated inference techniques on model that has a high representative power as well? Thus we will try to create a model which merges the advantages of both, MRFs and DNs to get even better results. There have been work that converted inconsistent dependency networks to markov networks \cite{lowdClosedFormLearningMarkov2012a}. Since we already have the better learned model, we can try to convert it to a different type of model for which, learning is hard but inference is fast and superior than dependency networks. }


\eat{
Sometimes dependency networks do not have valid distributions, but MRFs always correspond to a valid distribution. We will try to propose models which can take the advantages of both the models, the better representations from the DNs and better inference techniques from the MRFs. We can do the same by converting the better representations that we learn, to models on which we can do more sophisticated inferences. There have been work that converted dependency networks to markov networks \cite{lowdClosedFormLearningMarkov2012a}. }

==> misc/authors.tex <==
\author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
about author (webpage, alternative address)---\emph{not} for acknowledging
funding agencies.  Funding acknowledgements go at the end of the paper.} \\
Department of Computer Science\\
Cranberry-Lemon University\\
Pittsburgh, PA 15213, USA \\
\texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
\And
Ji Q. Ren \& Yevgeny LeNet \\
Department of Computational Neuroscience \\
University of the Witwatersrand \\
Joburg, South Africa \\
\texttt{\{robot,net\}@wits.ac.za} \\
\AND
Coauthor \\
Affiliation \\
Address \\
\texttt{email}
}

==> misc/keywords.tex <==
% Keywords. The author(s) should pick words that accurately describe the work being
% presented. Separate the keywords with commas.
\keywords{probabilistic graphical models, action classification,  multi-label classification, combining probabilistic models with deep learning, end-to-end learning}
